Gradient Descent Provably Optimizes Over-parameterized Neural Networks

One of the mysteries in the success of neural networks is randomly initialized first order methods like gradient descent can achieve zero training loss even though the objective function is non-convex and non-smooth. This paper demystifies this surprising phenomenon for two-layer fully connected ReLU activated neural networks. For an $m$ hidden node shallow neural network with ReLU activation and $n$ training data, we show as long as $m$ is large enough and no two inputs are parallel, randomly initialized gradient descent converges to a globally optimal solution at a linear convergence rate for the quadratic loss function. Our analysis relies on the following observation: over-parameterization and random initialization jointly restrict every weight vector to be close to its initialization for all iterations, which allows us to exploit a strong convexity-like property to show that gradient descent converges at a global linear rate to the global optimum. We believe these insights are also useful in analyzing deep models and other first order methods.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> multi_layer_regression.tex <==
In this section we show random initialized gradient flow converges to the global minimum for deep neural networks with ReLU activation.
Similar to Section~\ref{sec:two_layer_regression}, we first compute the time derivative of individual prediction.
\begin{align*}
	\frac{d}{dt}u_i= & \sum_{h=1}^{H} \sum_{r_{h}=1}^{d_h}\langle \frac{\partial u_i}{\partial \vect{w}_{r_h}^{(h)}}, \frac{d \vect{w}_{r_h}^{(h)}}{dt} \rangle \\
	= & \sum_{h=1}^{H}\sum_{r_h=1}^{d_h} \langle \frac{1}{\sqrt{d_H\cdots d_h}} \left[\vect{a}^\top \mat{J}_i^{(H)} \mat{W}^{(H)} \cdots \mat{J}_i^{(h+1) \mat{W}^{(h+1)} }\right]_{r_h} \vect{x}_i^{(h-1)} \indict\left\{(\vect{w}_{r_h}^{(h)})^\top \vect{x}_i^{(h-1)} \ge 0\right\} , \\
	&\sum_{j=1}^{n}(y_j-u_j) \frac{1}{\sqrt{d_H\cdots d_h}} \left[\vect{a}^\top  \mat{J}_j^{(H)} \mat{W}^{(H)}\cdots  \mat{J}_j^{(h+1)}\mat{W}^{(h+1)}\right]_{r_h} \vect{x}_j^{(h-1)} \indict\left\{(\vect{w}_{r_h}^{(h)})^\top \vect{x}_j^{(h-1)} \ge 0\right\} \rangle \\
	 = &\sum_{j=1}^{n}(y_j-u_j) \sum_{h=1}^{H} (\vect{x}_i^{(h-1)})^\top \vect{x}_j^{(h-1)} \sum_{r_h=1}^{d_h}\frac{\left[\vect{a}^\top \mat{J}_i^{(H)} \mat{W}^{(H)} \cdots  \mat{J}_i^{(h+1) \mat{W}^{(h+1)}}\right]_{r_h}
	 \left[\vect{a}^\top \mat{J}_j^{(H)} \mat{W}^{(H)} \cdots  \mat{J}_j^{(h+1) \mat{W}^{(h+1)}}\right]_{r_h}
	 	}{d_{H}\cdots d_h}\\ &\quad\cdot\indict\left\{(\vect{w}_{r_h}^{(h)})^\top \vect{x}_i^{(h-1)} \ge 0,(\vect{w}_{r_h}^{(h)})^\top \vect{x}_j^{(h-1)} \ge 0\right\} \\
	\triangleq &\sum_{j=1}^{n} (y_j-u_j) \sum_{h=1}^{H} G_{ij}^{(h)} 
\end{align*}
where we define \begin{align*}
G_{ij}^{(h)} = &(\vect{x}_i^{(h-1)})^\top \vect{x}_j^{(h-1)} \sum_{r_h=1}^{d_h}\frac{\left[\vect{a}^\top\mat{J}_i^{(H)}  \mat{W}^{(H)} \cdots  \mat{J}_i^{(h+1)} \mat{W}^{(h+1)}\right]_{r_h}
	\left[\vect{a}^\top \mat{J}_j^{(H)} \mat{W}^{(H)} \cdots  \mat{J}_j^{(h+1) \mat{W}^{(h+1)}}\right]_{r_h}
}{d_{H}\cdots d_h}\\ &\quad\cdot\indict\left\{(\vect{w}_{r_h}^{(h)})^\top \vect{x}_i^{(h-1)} \ge 0,(\vect{w}_{r_h}^{(h)})^\top \vect{x}_j^{(h-1)} \ge 0\right\} 
\end{align*}
We also define \begin{align*}
	\mat{G} = \sum_{h=1}^{H}\mat{G}^{(h)} \in \mathbb{R}^{n \times n}.
\end{align*}
We assume at the beginning $\lambda_{\min}(\mat{G}) \ge \lambda_0(n)$.
\simon{Note $\mat{G}^{(h)}(t)$ is positive semidefinite for all $h$ and $t$.
Thus alternatively, we can 	assume $\lambda_{\min}(\mat{G}^{(1)}(0)) = \lambda_0$ and only bounding perturbation on $\mat{G}^{(1)}(t)$.
	}

\begin{lem}\label{lem:small_perb_large_eigen}
If for $h \in [H]$, $r_h \in [d_h]$, $\norm{\vect{w}_{r_h}^{(h)}(t) - \vect{w}_{r_h}^{(h)}(0)}_2 \le R_h \triangleq$ \simon{to be determined}, we have \begin{align*}
\lambda_{\min}\left(\mat{G}(t)\right) \ge 
\end{align*}
\end{lem}
\begin{proof}[Proof of Lemma~\ref{lem:small_perb_large_eigen}]
We use perturbation analysis
\end{proof}

\begin{lem}\label{lem:large_eigen_small_perb}
If for all $0 \le s \le t$, $\lambda_{\min}(\mat{G}(s)) \ge \frac{\lambda_0}{2}$, we have for all $h \in [H]$, $r_h \in [d_h]$, 
$\norm{\vect{w}_{r_h}^{(h)}(t) - \vect{w}_{r_h}^{(h)}(0)}_2 \le R_h' \triangleq$. \simon{to be determined}
\end{lem}
\begin{proof}[Proof of Lemma~\ref{lem:large_eigen_small_perb}]
It is easy to show $\norm{\vect{y}-\vect{u}(t)}_2^2 \le \exp\left(-\lambda_0 t\right)\norm{\vect{y}-\vect{u}(0)}_2^2$.
It is easy to see if $\left[\frac{1}{\sqrt{d_H\cdots d_{ h+1}}} \vect{a}^\top \mat{J}^{(H)}\mat{W}^{(H)}  \cdots  \mat{J}^{(h+1)} \mat{W}^{(h+1)}\right]_{r_h}$ is $\tilde{O}(1)$ \simon{by perturbation or something...} and $\vect{x}_i^{(h)}$ is $O(1)$ then  we are fine because we can use the fact $\frac{1}{\sqrt{d_2}}$ to scale it down.
\end{proof}

\begin{lem}\label{lem:deep_contradiction}
	If for all $h \in [H]$, $R_h' < R_h$, we have for all $t$, $\lambda_{\min}(H(t)) \ge \frac{\lambda_0}{2}$ and for all $h \in [H]$, $r_h \in [d_h]$, 
	$\norm{\vect{w}_{r_h}^{(h)}(t) - \vect{w}_{r_h}^{(h)}(0)}_2 \le R_h'$.
\end{lem}
\begin{proof}[Proof of Lemma~\ref{lem:deep_contradiction}]
Standard argument.
\end{proof}



==> pre.tex <==
We consider an $H$-layer deep fully connected neural network.
%Suppose the input $\vect{x} \in \mathbb{R}^{d_0}$, $\mat{W}^{(1)} \in \mathbb{R}^{}$
 of the following form\begin{align}
f(\vect{x},\params,\vect{a}) = \frac{1}{\sqrt{d_Hd_{h-1}\cdot d_1}}\sum_{r_H=1}^{d_H} a_{r_H}\relu{
	\mat{W}^{(H)} \relu{
		\mat{W}^{(H-1)}\ldots \relu{\mat{W}^{(1)}\vect{x}}
		}
	}
\label{eqn:dnn_prediction}
\end{align}
where $\vect{x} \in \mathbb{R}^{d_0}$ is the input, $\mat{W}^{(h)} \in \mathbb{d_h \times d_{h-1}}$ is the weight at the $h$-th layer for $h = [H]$, $\relu{\cdot}$ denotes the rectified linear units (ReLU) and $\vect{a} \in \mathbb{R}^{d_H}$ is the output layer.

In this paper we focus the square loss \begin{align*}
L(\params) = \sum_{i=1}^{n}\frac{1}{2}\left(
f(\vect{x}_i,\params,\vect{a}) - y_i
\right)^2.
\end{align*}

Notation-wise, for convenience, we define \begin{align}
\vect{x}^{(h)} = \frac{1}{\sqrt{d_hd_{h-1}\cdot d_1}}\relu{
	\mat{W}^{(h)} \relu{
		\mat{W}^{(h-1)}\ldots \relu{\mat{W}^{(1)}\vect{x}}
	}
}\label{eqn:h_layer_output}
\end{align} as the input for the $(h+1)$-th layer.
Note this is equivalent to define $\vect{x}^{(h)}$ recursively \begin{align*}
\vect{x}^{(h)} = \frac{1}{\sqrt{d_h}} \relu{\mat{W}^{(h)}\vect{x}^{(h-1)}}.
\end{align*}
The scaling $1/\sqrt{d_h}$ plays an important role in our analysis.

Now we compute the derivative.
For $h \in [H]$, $r_h \in [d_{h}]$
\begin{align*}
	\frac{L(\params)}{\partial \vect{w}_{r_h}^{(h)}} = &\frac{1}{2}\sum_{i=1}^{n} \left(f(\vect{x}_i,\params,\vect{a})-y_i)\right)^2\\
=&\sum_{i=1}^{n}\left(f(\vect{x}_i,\params,\vect{a})-y_i)\right) \frac{\partial f(\vect{x}_i,\params,\vect{a})}{\partial \vect{w}_{r_h}^{(h)}} \\
= & \sum_{i=1}^{n}\left(f(\vect{x}_i,\params,\vect{a})-y_i)\right) \frac{\partial f(\vect{x}_i,\params,\vect{a})}{\partial x_{i,r_h}^{(h)}}  \cdot\frac{\partial x_{i,r_h}^{(h)}}{\partial \vect{w}_{r_h}^{(h)}} \\
= & \frac{1}{\sqrt{d_h}}\sum_{i=1}^{n}\left(u_i-y_i\right) \frac{\partial u_i}{\partial x_{i,r_h}^{(h)}}  \vect{x}_i^{(h-1)} \indict\left\{(\vect{w}_{r_h}^{(h)})^\top \vect{x}_i^{(h-1)} \ge 0 \right\}
\end{align*}
where \begin{align*}
\frac{\partial u_i}{\partial \vect{x}_i^{(h)}} = &\langle \vect{a}, \frac{\partial \vect{x}_i^{(H)}}{\partial \vect{x}_i^{(h)}} \rangle\\
=& \langle \vect{a}, \frac{\partial \vect{x}_i^{(H)}}{\partial \vect{x}_i^{(H-1)}} \cdots \frac{\partial \vect{x}_i^{(h+1)}}{\partial \vect{x}_i^{(h)}}  \rangle \\
=& \frac{1}{\sqrt{d_Hd_{H-1}\cdots d_{h+1}}}\langle \vect{a}, \mat{J}^{(H)}\mat{W}^{(H)}  \cdots \mat{J}^{(h+1)}\mat{W}^{(h+1)}  \rangle
\end{align*} where \[
\mat{J}^{(h')} \triangleq \diag\left(
\indict\left\{ (\vect{w}_{1}^{(h')})^\top \vect{x}^{(h'-1)}\ge 0 \right\}, \ldots,
\indict\left\{ (\vect{w}_{d_{h'}}^{(h')})^\top \vect{x}^{(h'-1)}\ge 0 \right\}
\right) \in \mathbb{R}^{d_{h'} \times d_{h'}}.
\]



==> technique.tex <==
In this section we present our analysis technique.
In Section~\ref{sec:linear_convergence_lr} we review when GD can achieve linear convergence on over-parameterized linear regression problem and identify the full-rankness of the Gram matrix is the key condition.
In Section~\ref{sec:random_features} we show because of the over-parameterization, the Gram matrix induced by the random initialization and ReLU  has full rank.
In Section~\ref{sec:overparams_stable}, we show over-parametrization also makes Gram matrix stable and so ensures the Gram matrix is full rank for all iterations.

\subsection{Review: Linear Convergence of Over-parameterized Linear Regression}
\label{sec:linear_convergence_lr}
We first review a simple setting, why gradient descent convergence linearly in over-parameterized linear regression model.
Suppose we have a data set $\left\{(\vect{x}_i,y_i)\right\}_{i=1}^n$ with $\vect{x}_i \in \mathbb{R}^d$and $d \ge n$.
We fit a linear model:\begin{align*}
	\min_{\vect{\theta} \in \mathbb{R}^d} L\left(\vect{\theta}\right) =  \frac{1}{2}\norm{\mat{X}\vect{\theta} - \vect{y}}_2^2
\end{align*}  where $\mat{X} = \left(\vect{x}_1,\ldots,\vect{x}_n\right)^\top \in \mathbb{R}^{n \times d}$ and $\vect{y} = \left(y_1,\ldots,y_n\right) \in \mathbb{R}^n$.
Now we apply gradient descent to optimize $\vect{\theta}$ \begin{align*}
	\vect{\theta}(k+1) = \vect{\theta}(k) - \eta \vect{X}^\top\left(\vect{X} \theta -\vect{y}\right).
\end{align*}
Note because we use over-parameterization: $n > d$, $\mat{X}^\top \mat{X}$ is \emph{not} full rank and so the objective function is not strongly convex.
However, if we look at the prediction space dynamics, we can show the linear convergence.
We denote $u_i = \vect{x}_i^\top \theta$ as the prediction on the $i$-th sample and compute \begin{align*}
u_i(k+1) = &\vect{x}_i^\top \theta\left(k+1\right) \\
= & u_i(k) - \vect{x}_i^\top \theta\left(k\right) - \eta \sum_{i=1}^{n} (\vect{x}_i^\top \vect{\theta}(k) - y_i)\vect{x}_i^\top \vect{x}_j \\
\triangleq
 \triangleq & u_i(k) - \sum_{j=1}^{n}(y_j-u_j(k))H_{ij}
\end{align*}
where we have defined $H_{ij} = \vect{x}_i^\top \vect{x}_j $.
Note if we view $H_{ij}$ as the $(i,j)$-th entry of an $n \times n$ matrix $\mat{H}$, it is just the Gram matrix.
Furthermore, because $n > d$, $\mat{H}$ is full-rank as long as the design matrix is not degenerate.
Denote $\vect{u} = \left(u_1,\ldots,u_n\right)$.
We can use $\mat{H}$ to obtain a compact form of the dynamics of $\vect{u}$\begin{align*}
\vect{u}(k+1) = \vect{u}(k) - \eta \mat{H}(\vect{y}-\vect{u}(k)).
\end{align*}
Thus we have \begin{align*}
\vect{y}-\vect{u}(k+1) = (1-\eta\mat{H})(\vect{y}-\vect{u}(k))
\end{align*} and we obtain the linear convergence dynamics \begin{align*}
\norm{\vect{y}-\vect{u}(k+1)}_2 \le (1-\eta\lambda_{\min}(\mat{H}))\norm{\vect{y}-\vect{u}(k)}_2
\end{align*} if the step size satisfies $\eta < \lambda_{\max}(\mat{H})$.
The key insight from this analysis is that as long as the Gram matrix $\mat{H}$ is full rank, we obtain the linear convergence on the prediction space.



\subsection{Features Generated by Random Initialization and ReLU}
\label{sec:random_features}
In this section, we consider an ideal setting in which 
we first randomly initialize $\mat{W}$ and $\vect{a}$, then use them to act on inputs $\vect{x}_i$s to generate  features and we fix these feature and optimize $\mat{W}$.
Specifically, for $\vect{x}_i$ we generate a new feature \[
\mat{X}_i' = \begin{pmatrix}\frac{1}{\sqrt{m}}
a_1 \indict\left\{(\vect{w}_1^{(0)})^\top \vect{x}_i \ge 0\right\} \vect{x}_i, \ldots, \frac{1}{\sqrt{m}}a_m \indict \left\{\left(\vect{w}_m^{(0)}\right)^\top \vect{x}_i\ge 0\right\}\vect{x}_i
\end{pmatrix} \in \mathbb{R}^{d \times m}.
\]
Once we fix the feature and because we only train $\mat{W}$ it becomes a linear regression problem\begin{align}
\widetilde{L}(\mat{W}) = \frac{1}{n}\sum_{i=1}^{n} \left(\langle\mat{W},\mat{X}_i'\rangle - y_i\right)^2 \label{eqn:loss_regression_rf}
\end{align}
The corresponding Gram matrix is \begin{align*}
	H_{ij} = &\vectorize{\vect{X}_i'}^\top \vectorize{\vect{X}_j'} \\
	= &\frac{1}{m} \sum_{r=1}^{m}a_r^2 \indict\left\{(\vect{w}_r^{(0)})^\top \vect{x}_i \ge 0 (\vect{w}_r^{(0)})^\top \vect{x}_j \ge 0\right\} \vect{x}_i^\top \vect{x}_j.
\end{align*}
This $H_{ij}$ is the $(i,j)$-th entry of Gram matrix $\mat{H}$.
We can call $\mat{H}$ a Gram matrix because we can view $H_{ij}$ inner product of the feature map that transforms an input $\vect{x}$ into $\vectorize{\mat{X'}}$.
If $a_r$ is sampled from a zero mean and unit variance distribution and $\vect{w}_r^{(0)}$ is sampled from Gaussian distribution with identity covariance, as $m \rightarrow \infty$
\begin{align*}
	H_{ij} \rightarrow \expect_{\vect{w} \sim N(\vect{0},\mat{I})}\left[\indict\left\{\vect{w}^\top \vect{x}_i \ge 0, \vect{w}^\top \vect{x}_j \ge 0\right\}\vect{x}_i^\top \vect{x}_j\right] = \frac{pi - \theta(\vect{x}_i,\vect{x}_j)}{2\pi} \vect{x}_i\vect{x}_j\triangleq H_{ij}^\infty.
\end{align*} where $\theta(\vect{x}_i,\vect{x}_j)$ is the angle between $\vect{x}_i$ and $\vect{x}_j$.
This $H_{ij}^\infty$ is the $(i,j)$-th entry of Gram matrix $\mat{H}^\infty$ as  $m \rightarrow \infty$.

Note in general, unless the data is degenerate, the smallest eigenvalue of $\mat{H}^\infty$ is strictly positive.
We refer readers to \cite{xie2017diverse} to a more detailed discussion of this matrix.
By standard concentration bounds, we can also bound the distance between $\mat{H}$ and $\mat{H}^\infty$.
Thus when $m$ is large, $\mat{H}$ is full rank and we still have the linear convergence rate for problem~\eqref{eqn:loss_regression_rf}.





\subsection{Over-parameterization Stabilizes Gram Matrix}
\label{sec:overparams_stable}
Different from loss function~\eqref{eqn:loss_regression_rf}, the Gram matrix induced by the original loss function~\eqref{eqn:loss_regression} is changing  because the feature map depends on $\mat{W}$ which is being updated at every iteration:\begin{align*}
	H_{ij}(k) = \frac{1}{m} \sum_{r=1}^{m}a_r^2 \indict\left\{(\vect{w}_r(k)^\top \vect{x}_i \ge 0, (\vect{w}_r(k)^\top \vect{x}_j \ge 0\right\} \vect{x}_i^\top \vect{x}_j.
\end{align*}
The first observation is this Gram matrix is stable with respect to the change of $\vect{w}_r$s because if $\abs{\vect{w}_r(0)^\top \vect{x}_i} \ge \gamma$ for some margin $\gamma$, only if $\abs{(\vect{w}_r(k)-\vect{w}_r(0))^\top \vect{x}_i} \ge \gamma$, the term \[a_r^2 \indict\left\{(\vect{w}_r(k)^\top \vect{x}_i \ge 0, (\vect{w}_r(k)^\top \vect{x}_j \ge 0\right\} \vect{x}_i^\top \vect{x}_j\] may change.
Furthermore, though some terms change, because of the normalization term $1/m$, they will only incur a small perturbation from $\mat{H}$.
Therefore, $\mat{H}(k)$ is still full rank if the perturbation is small.
We formalize this observation in Section~\ref{sec:two_layer_regression}.

Thus it is sufficient to show every $\vect{w}_r$ is close to it initialization.
First note that if the loss converges to $0$ with a linear rate (which can be guaranteed if $\mat{H}$ is always full rank), 
we can have  $
\sum_{k=0}^{\infty} \sqrt{L(\mat{W}(k))}  \le \kappa \sqrt{L\left(\mat{W}(0)\right)}
$  for some $\kappa > 0$ which is related to the specific convergence rate and independent of $m$.
We next examine the gradient of $\vect{w}_r$: \begin{align}
\norm{\frac{\partial L(\mat{W})}{\partial \vect{w}_r}}_2 = & \norm{\sum_{i=1}^n(f(\mat{W},\vect{a},\vect{x}_i)-y_i)\frac{1}{\sqrt{m}}a_r\vect{x}_i\indict\left\{\vect{w}_r(t)^\top \vect{x}_i \ge 0\right\} }_2 \nonumber\\
\le & \frac{\sqrt{n}}{\sqrt{m}}\sqrt{L(\mat{W})} \max_{r}\abs{a_r}\max_i\norm{\vect{x}_i}_2. \label{eqn:power_of_overparams}
\end{align} 
Using from Equation~\eqref{eqn:power_of_overparams}, we can bound the total deviation of a weight vector\begin{align*}
\norm{\vect{w}_r(k)-\vect{w}_r(0)}_2 \le &\sum_{k'=0}^{\infty} \norm{\frac{\partial L(\mat{W}(k'))}{\partial \vect{w}_r(k')}}_2 \\
\le & \frac{\sqrt{n}\kappa \sqrt{L(\mat{W}(0))} \max_{r}\abs{a_r}\max_i\norm{\vect{x}_i}_2}{\sqrt{m}}.
\end{align*}
From this inequality, it is easy to see if $m$ is large enough, the deviation is small.
The $\sqrt{m}$ in the denominator clearly demonstrates the power of over-parameterization.



